Scalable and Accurate Self-supervised Multimodal Representation Learning without Aligned Video and Text Data

Scaling up weakly-supervised datasets has shown to be highly effective in the image-text domain and has contributed to most of the recent state-of-the-art computer vision and multimodal neural networks. However, existing large-scale video-text datasets and mining techniques suffer from several limitations, such as the scarcity of aligned data, the lack of diversity in the data, and the difficulty of collecting aligned data. Currently popular video-text data mining approach via automatic speech recognition (ASR) used in HowTo100M provides low-quality captions that often do not refer to the video content. Other mining approaches do not provide proper language descriptions (video tags) and are biased toward short clips (alt text). In this work, we show how recent advances in image captioning allow us to pre-train high-quality video models without any parallel video-text data. We pre-train several video captioning models that are based on an OPT language model and a TimeSformer visual backbone. We fine-tune these networks on several video captioning datasets. First, we demonstrate that image captioning pseudolabels work better for pre-training than the existing HowTo100M ASR captions. Second, we show that pre-training on both images and videos produces a significantly better network (+4 CIDER on MSR-VTT) than pre-training on a single modality. Our methods are complementary to the existing pre-training or data mining approaches and can be used in a variety of settings. Given the efficacy of the pseudolabeling method, we are planning to publicly release the generated captions.

==> tables_algorithms/alg_separable_cross_att.tex <==
\begin{algorithm}[!t]
\caption{Separable Cross-Attention}
\label{alg:separable_cross_attention}
\textsc{Input:} $V \in \mathbb{R}^{s \times t \times h}$, $T \in \mathbb{R}^{l \times h}$, $W_{mix} \in \mathbb{R}^{h \times 2h}$ \\
\textsc{Output:} $a \in \mathbb{R}^{l \times h}$.\\

\begin{algorithmic}

\State $q = LayerNorm(T)$
\State $k_t = LayerNorm(\max_{s}{V})$ \Comment{Pool over space and normalize}
\State $a_t = Attention(q, k_t)$ \Comment{Attend over time}
\State $k_s = LayerNorm(\max_{t}{V})$ \Comment{Pool over time and normalize}
\State $a_s = Attention(q, k_s)$ \Comment{Attend over space}
\State $\hat a = W_{mix} [a_t:a_s]$ \Comment{Concatenate space and time attention and mix them}
\State $a = LayerNorm(\hat a + T)$ \Comment{Residual and normalize}\\
\Return $a$

\end{algorithmic}
\end{algorithm}

